Stackelberg Pricing is Hard to Approximate within $2-\epsilon$

Stackelberg Pricing Games is a two-level combinatorial pricing problem studied in the Economics, Operation Research, and Computer Science communities. In this paper, we consider the decade-old shortest path version of this problem which is the first and most studied problem in this family. The game is played on a graph (representing a network) consisting of {\em fixed cost} edges and {\em pricable} or {\em variable cost} edges. The fixed cost edges already have some fixed price (representing the competitor's prices). Our task is to choose prices for the variable cost edges. After that, a client will buy the cheapest path from a node $s$ to a node $t$, using any combination of fixed cost and variable cost edges. The goal is to maximize the revenue on variable cost edges. In this paper, we show that the problem is hard to approximate within $2-\epsilon$, improving the previous \APX-hardness result by Joret [to appear in {\em Networks}]. Our technique combines the existing ideas with a new insight into the price structure and its relation to the hardness of the instances.

==> algo.tex <==
\section{An Algorithm for Special Cases}

The gadgets we used are essentially the same as those used by Roch
et al and Joret, so it is interesting to see if this gadget can be
made strong enough to get a better hardness of approximation
result. We give a negative answer to the question by presenting a
$2$-approximation algorithm for all the hardness instances that
have ever appeared in the literature.

A {\em constraint satisfaction instance} $(P, F)$ consists of a
fixed cost path $P= (s=v_0, v_1, \ldots, v_m=t)$ from $s$ to $t$
where each edge $e_i=(v_{i-1},v_i)$ is associated with the fixed
cost $c_i
>0$. For each $i$, there are $n_i \geq 1$ {\em constraint paths}
from $v_{i-1}$ to $v_i$, and each constraint path $P^i_j$ ($1 \leq
j \leq n_i$) is of the form $P^i_j = (v_{i-1}, u^j_i, v^j_i,
v_{i})$ where $u^j_i v^j_i$ is a variable cost edge, while edges
$v_{i-1} u^j_i$ and $v^j_i v_{i}$ are fixed cost edges with zero
cost. Set $F$ contains shortcuts which are fixed cost edges of the
form $v^{j}_{i} u^{j'}_{i'}$. It is easy to see that this
definition captures the hardness instances in Roch et al, Joret,
and ours. Let $C= \sum_{i=1}^m c_i$. We prove the following
theorem.

\begin{theorem}
There is a polynomial time algorithm that, given a constraint
satisfaction instance, returns a price function that collects
revenue of at least $C/2$.
\end{theorem}

Since $C \geq \opt$, it follows immediately that we have a
$2$-approximation.

\begin{proof}
Initially, we set the price $p(e) = c_i/2$ for each variable cost
edge $e$ on constraint path $P^i_j$ for some $j$. Let $Q$ be a
resulting shortest path. 
\end{proof}


==> gap.tex <==
\section{Gap Analysis}\label{sec:analysis}

In this section, we show that the reduction gives a $(2-\eps)$-gap
between the case when $\phi$ is satisfiable and when it is not. In
section~\ref{subsection: yes instance}, we show that if $\phi$ is
satisfiable, then there is a price function that collects a revenue
of $M$. Section~\ref{subsection: no instance} shows that if $\phi$
is not satisfiable, there is no pricing strategy which collects
a revenue of more than $(1/2+\eps)M$.

\subsection{\yi}
\label{subsection: yes instance}

Let $f: \qset_1 \rightarrow \aset_1, \qset_2 \rightarrow \aset_2$
be an assignment that satisfies every constraint in $\Phi$. For
gadget $G_i$ corresponding to the variable $r_i$, set price $1$ to
the edge from $u^{a}_{i}$ to $v^{a}_{i}$ for $a= f(q_1(r_i))$.
Other edges are assigned the price of $\infty$.

Let $P$ be the shortest path on this graph w.r.t. the above
pricing. Notice that path $P$ does not contain any shortcut edge:
suppose there is a shortcut from $v^{a_i}_{i}$ to $u^{a_j}_{j}$ on
$P$. Since a shortcut only goes between two edges that represent
inconsistent assignments, then either $a_i$ is not consistent with
$a_j$ or $\pi_i(a_i)$ is not consistent with $\pi_j(a_j)$. We only
assign price $1$ to consistent assignments, so either the edge
entering $v^{a_i}_i$ or the one leaving $u^{a_j}_j$ has infinite
price, which contradicts the fact that $P$ is shortest path.

Since the shortcut is not used, the length of $P$ is exactly $M$,
and clearly there is a path from $s$ to $t$ collecting the
satisfied edges from every gadget. The total revenue is $M$.


\subsection{\ni}
\label{subsection: no instance}


We assume for contradiction that there is a pricing function which
collects a revenue of $(1/2+\eps) M$. Our goal is to construct an
assignment that satisfies more than $\eps M/3$ fraction of the
constraints in $\Phi$.

==== {\bf Bun:} We may remove it. === \\
==== I just don't want to start formal description so early in the
section. ====

%Before proceeding to the formal explanation, we will briefly explain
%the idea for constructing an assignment from a given pricing
%function. Assume that $P$ is a shortest path from the first gadget to
%the last gadget that yields maximum revenue. One can obtain an
%assignment by setting $x_e=1$ for a variable cost edges that has
%non-zero price and setting $x_e=0$, otherwise. However, the assignment
%may not be feasible because there might be some short-cut edges in the 
%path which cause conflict in the assignment. Thus, the main task is to
%recover an assignment from a shortest path. 

%The key idea of our construction is to decompose a path into subpaths in
%such a way that no path contain head and tail of shortcut-edges. The
%construction guarantees that the number of gadget throwing out is not
%so much and, thus, we can recover more than some fraction of the
%max-revenue. We will now proceed to the formal description.

To ensure that there is no conflict in the decoded assignment, we have
to decompose a max-revenue shortest path $P$ into subpaths in such a
way that no short-cut edge joining two subpaths. Hence, we can
independently setting the variables corresponding to each subpath
without creating a conflict.

======================================================

A subpath $Q \sse P$ is said to be a {\em source-sink subpath} if
it starts at some source $s_i$ and ends at some sink $t_j$ for $i
\leq j$. Let $Q$ be a source-sink subpath. From now on, unless
stated otherwise, we will look at path $Q$ as a set of edges. Let
$\sset = \set{Q_1,\ldots, Q_k}$ be a set of source-sink subpaths
of path $Q$. We say that $\sset$ is a {\bf *source-sink partition*} of
path $Q$ if $Q \setminus (\bigcup_{j=1}^k Q_j)$ contains no
variable cost edges. In other words, every variable cost edge
appears in some paths in $\sset$. The following theorem is the key
idea to proving the result.

\begin{theorem}[Path Decomposition]
\label{theorem: path decomposition} Let $P$ be a shortest path in
the graph. Then we can find, in polynomial time, sets $\rset,
\rset'$ such that the following properties hold.

\renewcommand{\theenumi}{D\arabic{enumi}}

\be

\item \label{property: partition} $\rset \cup \rset'$ is a
source-sink partition of $P$.

\item \label{property: small revenue in R'} The revenue collected
from edges on paths in $\rset'$ is at most $M/2 + O(1)$.

\item \label{property: small edge revenue} Let $e$ be a variable
cost edge in $\rset$. Then the price of $e$ is at most $1$.

\item \label{property: no constraint} Let $e, e'$ be two variable
cost edges in $\rset$. Then there is no shortcut between $e$ and
$e'$.

\ee

\end{theorem}

We defer the proof of this theorem to the next section. Meanwhile
we show how the theorem implies that we can construct an
assignment that satisfies more than $\eps/3$ fraction of the
constraints in $\Phi$, thus a contradiction. Since we can collect
a revenue of at most $M/2 + O(1) < M/2+ \eps M/3$ from edges in
$\rset'$, at least $2 \eps M/3$ must be collected from edges in
$\rset$. We let $E'$ contain all edges that lie on some path in
$\rset$. From the third property, we have $\abs{E'} \geq 2\eps
M/3$. Let $F \sse E'$ be the set of edges that lie in far gadget.
Recall that we have at most $\eps M/3$ gadgets that are not far,
so $\abs{F} \geq \eps M/3$. We are now ready to describe how we
get an assignment that satisfies a large fraction of constraints
in $\Phi$. For each edge $e \in F$, edge $e$ can be written as
$u^{a_i}_{i}, v^{a_i}_i$ for some gadget $i$. We assign the value
of $a$ to $q_1(r_i)$ and $\pi_i(a)$ to $q_2(r_i)$. This assignment
will definitely satisfy the constraint $r_i$. This process
satisfies at least $\eps M/3$ constraints corresponding to edges
in $F$ provided that there is no conflict in assignment. We argue
that there is no such conflict. Assume that the above process
creates a conflict assignment to the same query $q$. This means
that there are two constraints $r_i, r_j \in \Phi$ for $i <j$ with
$q=q_1(r_i) =q_1(r_j)$ (the other case can be proved similarly),
and such query $q$ were assigned different answers when processing
gadgets $i$ and $j$. Since they are both far gadgets, by
construction, there must be a shortcut between two vertices. This
contradicts the fact that there is no shortcut in $\rset$.

\subsection{Proof of Theorem~\ref{theorem: path decomposition}}

Denote by $s(Q)$ and $t(Q)$ the gadget index to which the source
and sink of $Q$ belong respectively. Since there is a fixed-cost
path of length $t(Q) - s(Q) +1$ from $s_{s(Q)}$ to $t_{t(Q)}$, the
revenue collected on $Q$ is at most $t(Q)-s(Q)+1$, which will be
denoted by $\len(Q)$. We let $\rev(Q)$ be the revenue collected on
subpath $Q$, i.e. $\rev(Q) = \sum_{e\in Q\cap E_v} p(e)$. We first
state the following lemma whose proof is obvious.

\begin{lemma}
If $\sset=\set{Q_1,\ldots, Q_k}$ be a {\bf *source-sink partition*} of
$Q$, then 
\[\sum_{j=1}^k \len(Q_j) = \len(Q) \]
\end{lemma}

%We will decompose $P$ into a number of source-sink subpaths and
%add them into three separated sets, $\rset, \sset$ and $\tset$
%where $\sset$ and $\tset$ are supposed to contain all the
%source-sink subpaths $Q$ from which at most roughly $\len(Q)/2$
%can be collected and $\rset$ is supposed to get $\geq
%\len(\rset)/2+\eps M$ (TO BE RESTATED).

Our decomposition has two phases. Initially, $\rset=\{P\}$, and
$\sset=\tset=\emptyset$. In the first phase, we remove the portion
of paths $P$ which contains the shortcut edges and add them to set
$\tset$. We ensure that paths are always cut into source-sink
subpaths. The set $\rset'$ in the theorem is just $\tset \cup
\sset$.

%Then we deal with the subpaths that will give an inconsistent
%assignment, removing them from $\rset$ and adding them in $\sset$.
%Our $\rset'$ in the theorem is formed by $\rset' = \sset \cup
%\tset$. We are ready to begin the description of the
%decomposition.


\paragraph{Phase 1:} Initially, $\rset= \set{P}$ and $\tset = \emptyset$.
%While
%there is a shortcut $(v,v')$ used by some path $P' \in \rset$, we do
%the following.
While there exists a path $P'\in \rset$ that contains a shortcut
edge, do the following. Let $vv'$ be any shortcut edge. Let $s'$
be the last source vertex that appears before $v$ in $P'$ and let
$t'$ be the first sink vertex that appears after $v'$ in $P'$.
First remove $P'$ from $\rset$. Denote by $Q$ the source-sink
subpath of $P'$ from $s'$ to $t'$. We break $P'$ into at most
three source-sink subpaths $Q_l$, $Q$, and $Q_r$ where $Q_l$ ends
at vertex $s'$, $Q$ starts and ends at $s'$ and $t'$ respectively,
and $Q_r$ starts and $t'$.
%We remove the subpath $Q$ from $P'$, thus breaking the path $P'$
%into at most three valid subpaths $Q_l, Q, Q_r$.
We then add $Q$ to $\tset$ and add $Q_l,Q_r$ back to $\rset$.


%\paragraph{Phase 1:} Initially, $\rset= \set{P}$ and $\tset = \emptyset$. While
%there is a shortcut $(v,v')$ used by some path $P' \in \rset$, we
%do the following. First remove $P'$ from $\rset$. Let $S_i$ be the
%last source of gadget $i$ on $P'$ to which $v$ is reachable, and
%$T_j$ be the first sink reachable from $v'$ on $P'$. Denote by $Q$
%the valid subpath of $P'$ from $S_i$ to $T_j$. We remove the
%subpath $Q$, thus breaking the path $P'$ into at most three valid
%subpaths $Q_l, Q, Q_r$. We then add $Q$ to $\tset$ and add
%$Q_l,Q_r$ back to $\rset$.

Consider the set $\rset' = \sset \cup \tset$. We show that, after
this phase, the output satisfies properties~\ref{property:
partition}, \ref{property: small revenue in R'}, and
\ref{property: small edge revenue}. In the second phase, we will
ensure property~\ref{property: no constraint} while other
properties remain to hold. It is easy to see that
property~\ref{property: partition} holds. The next two lemmas
prove property~\ref{property: small edge revenue} and
\ref{property: small revenue in R'}.

\begin{lemma}
\label{lemma: limited revenue per gadget} After Phase 1, let $e
\in E_v$ be an edge that belongs to some path $Q \in \rset$. Then
$p(e) \leq 1$.
\end{lemma}

\begin{proof}
This is the case just because path $Q$ is a source-sink subpath.
Recall that edge $e$ can be written in the form $u^a_i v^a_i$ for
some $i,a$. Since path $Q$ is a source-sink subpath, vertices
$s_i$ and $t_i$ also belong to $Q$. If $p(e)
>1$, the shortest path would have used the edge $s_i t_i$ instead.
\end{proof}

We will need the following claim to prove property~\ref{property:
small revenue in R'}.

\begin{claim}
\label{claim: limited revenue in T} For each path $Q \in \tset$,
we have $\rev(Q) \leq (\len(Q)+1)/2$
\end{claim}

\begin{proof}
Consider path $Q \in \tset$ from $s_i$ to $t_j$. Recall that there
is a path of length $\len(Q)$ in $G$ from $s_i$ to $t_j$, so
$\rev(Q) \leq \len(Q)$. It is therefore sufficient to prove that
the total cost of the shortcuts on $Q$ is at least
$(\len(Q)-1)/2$. The way we construct paths in $\tset$ guarantees
that path $Q$ must be of the form
\[s_i \rightarrow u^{a_1}_{i_1}\rightarrow v^{a_1}_{i_1} \rightarrow
u^{a_2}_{i_2}\rightarrow \ldots \rightarrow v^{a_q}_{i_q}
\rightarrow t_j\]

where $i_1= i, j_x= j$, and edges of the form $u^{a_x}_{i_x}
\rightarrow v^{a_{x}}_{i_{x}}$ are the variable cost edges, from
which we can collect a revenue. Other
 edges of the form $v^{a_x}_{i_x}
\rightarrow u^{a_{x+1}}_{i_{x+1}}$, for $1 \leq x <q$, are
shortcuts. Hence the total cost of shortcuts can be written as a
telescopic sum, $\sum_{x=1}^{q-1}
\paren{\frac{i_{x+1}-i_x}{2}} = (j-i)/2=(\len(Q)-1)/2$.
\end{proof}

\begin{lemma}
\[\sum_{Q \in \tset} \rev(Q) \leq  \frac{1}{2}\paren{\sum_{Q \in \tset} \len(Q)} + O(1/\delta) \]
In particular, after the first phase, the revenue in $\rset'$ is
at most $M/2+ O(1)$.
\end{lemma}

\begin{proof}
From Claim~\ref{claim: limited revenue in T}, it follows
immediately that
\[\sum_{Q \in \tset} \rev(Q) \leq \sum_{Q \in
\tset} \paren{\len(Q)/2 + 1/2} \leq \frac{1}{2}\paren{\sum_{Q \in
\tset} \len(Q)}+ \abs{\tset}/2 \]

It then suffices to bound the size of set $\tset$ by
$O(1/\delta)$. Notice that each path in $\tset$ contains at least
one shortcut edge. Since each shortcut edge only goes from $v^a_i$
to $u^{a'}_j$ if $\abs{j-i} \geq \delta M$ and the intervals in
the set $\set{[s(Q), t(Q)]: Q \in \tset}$ are disjoint, we can
have at most $O(1/\delta)$ paths in $\tset$.
\end{proof}


%Since we assume that we can collect $(1/2+\eps)M$, at least $\eps
%M$ of the revenue must be collected from paths in the set $\rset$.
%Let $E' \sse E_v$ be the set of variable cost edges on some paths
%in $\rset$ from which positive revenue is collected, and $V'$ be
%the set of vertices appearing in $E'$. Due to
%observation~\ref{claim: limited revenue per gadget}, we have
%$\abs{E'} \geq \eps M$. If there is no shortcut $vv'$ for $v, v'
%\in V'$, we immediately get an assignment satisfying
%$\eps$-fraction of the constraints in $\Phi$ (and thus a
%contradiction): each edge in $E'$ tells how the assignment can be
%chosen for each query $q$, and if there is no shortcut, all such
%assignments are consistent. Unfortunately, there can be shortcuts
%in $\rset$, and that is why we need the second phase.

\paragraph{Phase 2:} Initially, we have $\rset$ and $\tset$ from Phase
1, and $\sset =\emptyset$. We proceed in iterations starting from
iteration $1$. Here is the description of iteration $i$:

\bi

\item We first check if source $s_i$ belongs to some path in
$\rset$. If not, we proceed to iteration $i+1$.

\item If $S_i$ does belong to some path $Q$ in $\rset$, we then
check if there is a shortcut edge (that, of course, does not lie
on to $Q$) leaving $B_{(i,b,b')} \in Q$ to some vertex
$A_{(j,a,a')}$ on some path $Q' \in \rset$. Note that $Q$ and $Q'$
may be the same. Let $P' \sse P$ be the source-sink subpath from
$S_i$ to $T_j$. There are two possible cases for $P'$.

    \be
         \item If $Q$ and $Q'$ are the same path, then $P' \sse Q$. We
remove $Q$ from $\rset$. Break $Q$ into at most three source-sink
subpaths $Q_l P' Q_r$. Add $P'$ to $\sset$, and add $Q_l, Q_r$ to
$\rset$.

         \item Notice that when $Q \neq Q'$, path $P'$
contains subpaths from both $\rset$ and $\tset$. In this case, we
first remove $Q$ and $Q'$ from $\rset$. We also remove from
$\rset$ and $\tset$, every path that is a subpath of $P'$. We add
$Q \setminus P'$ and $Q'\setminus P'$ back to $\rset$ (notice that
both of them are source-sink subpaths). And add $P'$ to set
$\sset$. After this step is performed, we can proceed to iteration
$j+1$ since everything between gadget $i$ to $j$ is already
removed from $\rset$.


    \ee
\ei


We first check that properties \ref{property: partition} and
\ref{property: small edge revenue} still hold after this phase.
Property~\ref{property: partition} is trivial. Since paths in
$\rset$ only get chopped off, Lemma~\ref{lemma: limited revenue
per gadget} still holds, and thus property~\ref{property: small
edge revenue}. The next claim shows property~\ref{property: no
constraint}.

\begin{claim}
After Phase 2, there is no shortcut between any two subpaths in
$\rset$.
\end{claim}

\begin{proof}
Notice that once a shortcut leaving gadget $i$ is found, the whole
part of gadget $i$ is removed completely from $\rset$. Therefore
it is easy to see that the following holds. After iteration $i$,
there is no shortcut leaving vertex in $P \cap G_i$ to other
vertices lying on some path in $\rset$.
\end{proof}


Similarly to Claim~\ref{claim: limited revenue in T}, we can also
bound the revenue on paths in $\sset$.

\begin{claim}
\label{claim: limited revenue in S} For each path $Q \in \sset$,
we have $\rev(Q) \leq \frac 1 2 \len(Q) + 2$
\end{claim}

\begin{proof}
Consider path $Q \in \sset$ from $s_i$ to $t_j$. Path $Q$ can be
written in the form: \[s_i \rightarrow u^{a_i}_i \rightarrow
\ldots \rightarrow v^{a_j}_j \rightarrow t_j\] Let $Q'$ be the
subpath of $Q$ from $v^{a_i}_i$ to $u^{a_j}_j$, and $e_i, e_j$ be
the edges $u^{a_i}_i v^{a_i}_i$ and $u^{a_j}_j v^{a_j}_j$
respectively. Then $Q = s_i e_i Q' e_j t_j$. The revenue collected
on $Q$ either comes from edges in $Q'$ or from $e_i$ and $e_j$.
Since both $e_i$ and $e_j$ belonged to $\rset$ after Phase 1, we
have $p(e_i) + p(e_j) \leq 2$. Path $Q'$ can collect a revenue of at
most $(j-i)/2$ due to the fact that there is a shortcut edge
$v^{a_i}_i u^{a_j}_j$ of cost $(j-i)/2$. Overall the revenue on
$Q$ is at most $(j-i)/2+2 < \len(Q) + 2$.
\end{proof}


\begin{lemma}
\[\sum_{Q \in \sset} \rev(Q) \leq  \frac{1}{2}\paren{\sum_{Q \in \sset} \len(Q)} + O(1/\delta) \]
\end{lemma}
\begin{proof}
Since there is a shortcut edge in every path $Q \in \sset$, the
length of such path is at least $\delta M$. Therefore,
$\abs{\sset} \leq O(1/\delta)$. We invoke Claim~\ref{claim:
limited revenue in S} for every path in $\sset$ and sum them up.
This immediately gives the lemma.
\end{proof}


==> open.tex <==
\section{Open problems and discussion}
Throw a lot of open problems here. 

